Bagging, optimized dynamic mode decomposition (BOP-DMD) for robust, stable forecasting with spatial and temporal uncertainty-quantification

Dynamic mode decomposition (DMD) provides a regression framework for adaptively learning a best-fit linear dynamics model over snapshots of temporal, or spatio-temporal, data. A diversity of regression techniques have been developed for producing the linear model approximation whose solutions are exponentials in time. For spatio-temporal data, DMD provides low-rank and interpretable models in the form of dominant modal structures along with their exponential/oscillatory behavior in time. The majority of DMD algorithms, however, are prone to bias errors from noisy measurements of the dynamics, leading to poor model fits and unstable forecasting capabilities. The optimized DMD algorithm minimizes the model bias with a variable projection optimization, thus leading to stabilized forecasting capabilities. Here, the optimized DMD algorithm is improved by using statistical bagging methods whereby a single set of snapshots is used to produce an ensemble of optimized DMD models. The outputs of these models are averaged to produce a bagging, optimized dynamic mode decomposition (BOP-DMD). BOP-DMD not only improves performance, it also robustifies the model and provides both spatial and temporal uncertainty quantification (UQ). Thus unlike currently available DMD algorithms, BOP-DMD provides a stable and robust model for probabilistic, or Bayesian forecasting with comprehensive UQ metrics.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
%\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
%\else
%  \DeclareGraphicsExtensions{.eps}
%\fi

\graphicspath{{figures/}{BrBuKaKu_SIAMReview/figures/}{BrBuKaKu_SIAMReview/}}
%strongly recommended
\numberwithin{theorem}{section}

% Declare title and authors, without \thanks
%\newcommand{\TheTitle}{Modern Koopman Operator Theory\\ for Data-Driven Dynamical Systems}
\newcommand{\TheTitle}{Modern Koopman Theory for Dynamical Systems}
\newcommand{\TheAuthors}{S. L. Brunton, M. Budi\v{s}i\'{c}, E. Kaiser, J. N. Kutz}

% Sets running headers as well as PDF title and authors
\headers{\TheTitle}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}\thanks{Submitted to the editors Feb. 24, 2021.
\funding{
SLB acknowledges support from the Army Research Office (W911NF-17-1-0306 and W911NF-19-1-0045).
SLB and JNK acknowledge support from the Defense Advanced Research Projects Agency (DARPA contract HR011-16-C-0016) and the UW Engineering Data Science Institute, NSF HDR award \#1934292.
}}}

% Authors: full names plus addresses.
\author{
  \hspace{-.1in}Steven L. Brunton\thanks{Dept. of Mechanical Engineering, University of Washington, Seattle, WA (\email{sbrunton@uw.edu}).}
  \and
    Marko Budi\v{s}i\'{c}\thanks{Dept. of Mathematics, Clarkson University, Potsdam, NY (\email{mbudisic@clarkson.edu}).}
  \and
    Eurika Kaiser\thanks{Dept. of Mechanical Engineering, University of Washington, Seattle, WA  (\email{eurika@uw.edu}).}
  \and
  J. Nathan Kutz\thanks{Dept. of Applied Mathematics, University of Washington, Seattle, WA (\email{kutz.edu}).  \hspace{-.1in}}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}




%%% Local Variables:
%%% mode:latex
%%% TeX-master: "main"
%%% End:

